Expert-augmented actor-critic for ViZDoom and Montezumas Revenge

We propose an expert-augmented actor-critic algorithm, which we evaluate on two environments with sparse rewards: Montezumas Revenge and a demanding maze from the ViZDoom suite. In the case of Montezumas Revenge, an agent trained with our method achieves very good results consistently scoring above 27,000 points (in many experiments beating the first world). With an appropriate choice of hyperparameters, our algorithm surpasses the performance of the expert data. In a number of experiments, we have observed an unreported bug in Montezumas Revenge which allowed the agent to score more than 800,000 points.

==> experiments.tex <==
% \subsection{Montezuma's Revenge}

% We use our Expert-augmented ACKTR algorithm, recall Algorithm \ref{listing} to train an agent playing Montezuma's Revenge. We choose future discounted reward as expert advantage
% estimate, conjecturally this excludes suboptimal expert actions leading to agent's loss
% of life.  We repeat the experiment with 3 random seeds. 


% We perform an experiment where Expert-augmented ACKTR is used to play
% Montezuma's Revenge. We choose future discounted reward as expert advantage
% estimate in order to exclude suboptimal expert actions leading to agent's loss
% of life. We stop training every hour of wall time in order to run evaluation,
% results of which are presented in Figure \ref{monte-3-eval}. We repeat the
% experiment with 3 random seeds to get better estimates of performance
% statistics.


% The agent reaches the average reward of 6560 points and median 8000 after training on 200M frames. The results are presented in Figures
% \ref{monte-3-train} and \ref{monte-3-eval}. Our method is more sample
% efficient than previous methods, such as DQfD
% \cite{DQfD} that reaches 4739.6 points in 200M frames\todo{Looks like a poor marketing. We use the same number of samples but claim that we are more "sample efficient"? It sounds like an add of a car A which says it is more economical than car B, because it uses 10l of gas per 100 kilometer, but the car B also uses 10l of per 100 kilometer. Maybe we should just underline that we are getting better average and median? }. Our agent consistently explores most of
% the rooms of the first world, as depicted in Figure
% \ref{exploredrooms}. In \href{https://www.youtube.com/playlist?list=PL1dkNgD0lNRavH4np0AQNY5SnBrTSCfzC}{videos} we present a selection of evaluation rollouts. We observed that often the trained actor
% is not able to get through a particularly tricky central room and therefore is
% stuck on score of 8000. To resolve this issue we run experiments with random starting points as described in the next paragraph.

% The agent reaches the average reward of 6560 points and median 8000 after training on 200M frames. The results are presented in Figures
% \ref{monte-3-train} and \ref{monte-3-eval}. Our results are more sample
% efficient than previous results of previous comparable methods, such as DQfD
% \cite{DQfD} that reach 4739.6 points in 200M frames. Our agent consistently explores most of
% the rooms of the first world, as depicted in Figure
% \ref{exploredrooms}. We
% \href{https://www.youtube.com/playlist?list=PL1dkNgD0lNRavH4np0AQNY5SnBrTSCfzC}{link
% a playlist}, where we present videos of a variety of stronger evaluation runs
% of our algorithm.  Qualitatively, it is very often the case the trained actor
% is not able to get through a particularly tricky central room and therefore is
% stuck on score of 8000. This obstacle is cleared in the next section at the
% cost of requiring ability to set the state of the environment.
\todo[inline]{pm: do we really want to cite dqn here?}
In comparison, standard non-augmented A2C and ACKTR fail to produce any decent results in Montezuma's Revenge.\todo{In our experiments or in general? If in general, then we should add a citation.}
Further, supervised learning from the expert data yields average score of 570 in \cite{DQfD}. 
\todo[inline]{Overall heuristic is that this kind of data should be in a table. Inlining makes it hard to read}%Taking into account that the expert training data is near-optimal, this is surprisingly weak result.

% In comparison, actor-critic methods such as A2C and ACKTR without additional modules promoting exploration do not learn anything useful in this setting. Further, supervised learning of expert data yields average score of 570 in \cite{dqn} and we report evaluation scores of below 400 in the same setup. Taking into account that the expert training data is near-optimal, this is surprisingly weak result.


\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
                \includegraphics[scale=0.5]{monte-3-train.png}
                \caption{Training}
        \label{monte-3-train}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.5\textwidth}
    \centering
        \includegraphics[scale=0.5]{monte-3-eval.png}
                                \caption{Evaluation}
                        \label{monte-3-eval}
    \end{subfigure}
    \caption{Montezuma's Revenge. Mean and median rewards in evaluation achieved by one parametrization of our method over 3 random seeds.}
\end{figure*}

% \todo[inline]{Figures in figure 4 and other figures, must be {\bf precisely} aligned - otherwise looks amateurishly}

 \begin{minipage}{\linewidth}
  \centering
\begin{figure}[H]
        \centering
        \includegraphics[scale=0.35]{explored_rooms.png}
        \caption{Rooms explored during a sample evaluation of our agent.}
        \label{exploredrooms}
\end{figure}
\end{minipage}
  
  
  % As a check of robustness to the choice of parameters we present the training performance of the algorithm over the grid of parameters on the below Figure \ref{monte-grid-train}.

% The parameters checked were learning rate, entropy coefficient, future discount factor $gamma$, and type of expert advantage estimate. 
% \todo{More details here}

% \begin{minipage}{\linewidth}
%   \centering
% \begin{figure}[H]
%       \centering
%       \includegraphics[scale=0.6]{monte-grid-train.png}
%       \caption{Training environment reward at the end of epsiode. The line in the middle represents the average, the inner shaded area 25th and 75th percentiles, the outer shaded ares minimum and maximum.}
%       \label{monte-grid-train}
% \end{figure}
%   \end{minipage}



\paragraph{Experiments with expert state resets}
\todo[inline]{pm: I've removed for now the note about the sample complexity. It seems somewhat not clear}
As episodes always start from the same position, the beginning of the game is overrepresented in training. To alleviate this, we start episodes from a state drawn uniformly from the states visited in expert trajectories. We repeat the experiment with two random seeds. \todo[inline]{It would be great if we can make it 10 random seeds in all places}

The results of this experiments can be seen in Figures \ref{monte-starts-train} and \ref{monte-starts-eval}. Note that the training results are from random starting state, thus are not comparable with the previous results. In the evaluation we use the original starting point. Interestingly, the  agent trained this way is often able to complete the whole first world, scoring 44 000 points, see \href{https://www.youtube.com/playlist?list=PL1dkNgD0lNRb4zAGzX0VJGbX3gMfsmVK6}{videos}. The drawback is that training is less stable, the reason of that is yet to be investigated. 

% This method

% This results in general slow-down of training in terms of sample efficiency, however it unlocks occasional very good evaluations. The approach presented reliably produces runs where 200M training frames is enough to generate policy that has relatively high variance, but occasionally produces very strong evaluations that solve the first world of the game.
% \href{https://www.youtube.com/playlist?list=PL1dkNgD0lNRb4zAGzX0VJGbX3gMfsmVK6}{Here} we present such cherry-picked very strong evaluations.

% As eposodes always start from the same position, the beginning of the game is overrepresented in training. In order to  alleviate this, we introduce a mechanism in which environment is restored to a state drawn uniformly from the distribution of states visited in expert trajectories.

% This results in general slow-down of training in terms of sample efficiency, however it unlocks occasional very good evaluations. The results of this experiments can be seen in Figures \ref{monte-starts-train} and \ref{monte-starts-eval}. The approach presented reliably produces runs where 200M training frames is enough to generate policy that has relatively high variance, but occasionally produces very strong evaluations that solve the first world of the game.
% \href{https://www.youtube.com/playlist?list=PL1dkNgD0lNRb4zAGzX0VJGbX3gMfsmVK6}{Here} we present such cherry-picked very strong evaluations.


% \todo[inline]{Figures (a) and (b) must be separated or change to have similar size. The white space above (a) is not acceptable. }


\begin{figure}[H]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
                        \includegraphics[scale=0.45]{monte-starts-train.png}
                        \caption{Training.}
                        \label{monte-starts-train}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.5\textwidth}
    \centering
\includegraphics[scale=0.45]{monte-starts-eval.png}
                        \caption{Evaluations}
                        \label{monte-starts-eval}
    \end{subfigure}
    \caption{Montezuma's Revenge. Mean and median rewards in evaluation achieved by one parametrization of our method over 2 random seeds.}
\end{figure}


\subsection{Vizdoom}

\paragraph{\MyWayHomeVerySparse}
% \todo[inline]{pm: In this case we use
%simple expert advantage estimate, which is equivalent to supervised
%``classification``  of expert advantage. What does it mean????????}
%We experiment with a deterministic version of the above \MyWayHome environment,
%introduced by \cite{curiosity}, in which the agent is always spawned in the
%room that is furthest from the reward, see Figure \ref{doom-map}. This version is particularly hard for non-expert augmented methods, as
%random exploration is extremely unlikely to find any reward. In this case we use
%simple expert advantage estimate, which is equivalent to supervised
%``classification``  of expert advantage. We repeat our experiments with two random seeds. 
The results of our experiments are presented on Figures \ref{doom-very-sparse-eval} and \ref{doom-very-sparse-train}. Expert-augmented ACKTR, Algorithm \ref{listing}, is very efficient in this setting, achieving perfect performance in just 5 million frames, corresponding to only one hour of training, see \href{https://www.youtube.com/playlist?list=PL1dkNgD0lNRYq0PuPVX9i4-mQ2AWVwM8N}{videos}. In comparison, both behavioral cloning of expert transitions and vanilla
actor-critic fail to learn anything useful. 


\begin{figure}[H]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
                \includegraphics[scale=0.45]{doom-very-sparse-both-eval.png}
                \caption{Evaluation. Each bar represents 5 evaluation runs.}
                       \label{doom-very-sparse-eval}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
                \includegraphics[scale=0.45]{doom-very-sparse-train.png}
                \caption{Training}
                \label{doom-very-sparse-train}
    \end{subfigure}
    \caption{
        \MyWayHomeVerySparse.
        Mean and median evaluation rewards and training rewards for
        2 runs with different random seeds.
    }
\end{figure}


\paragraph{\MyWayHome}
We compare standard ACKTR with Expert-augmented ACKTR on standard \MyWayHome
which has significantly denser rewards.  In this case both methods obtain
similar results. ACKTR deals with this
environment relatively well, as actor is spawned uniformly over the whole
space, sometimes getting spawned close to the goal, helping to gradually infer
the optimal policy. As shown in Figures \ref{doom-vanilla-eval} and
\ref{doom-expert-eval}, expert data reduce slightly the sample complexity, reaching perfect
evaluation in 150M frames as opposed to 175M frames needed by method
without expert data.

\begin{figure}[H]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[scale=0.5]{doom-expert-train.png}
        \caption{With expert data.}
        \label{doom-expert-train}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[scale=0.5]{doom-vanilla-train.png}
        \caption{Without expert data.}
        \label{doom-vanilla-train}
    \end{subfigure}
    \caption{
        Vizdoom MyWayHome.
        Average training enviroment rewards averaged over 2 random seeds.
    }
\end{figure}

\begin{figure}[H]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[scale=0.5]{doom-expert-eval.png}
        \caption{With expert data}
        \label{doom-expert-eval}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[scale=0.5]{doom-vanilla-eval.png}
        \caption{Without expert data}
       \label{doom-vanilla-eval}
    \end{subfigure}
    \caption{
        Vizdoom MyWayHome.
        Mean and median evaluation, averaged over 2 random seeds.
        Each bar represents 5 evaluation runs.
    }
\end{figure}

